Dispersing Fermi-Ulam Models

We study a natural class of Fermi-Ulam Models that features good hyperbolicity properties and that we call dispersing Fermi-Ulam models. Using tools inspired by the theory of hyperbolic billiards we prove, under very mild complexity assumptions, a Growth Lemma for our systems. This allows us to obtain ergodicity of dispersing Fermi-Ulam Models. It follows that almost every orbit of such systems is oscillatory.

==> fum-p.tex <==
% multiple inclusion guard
\makeatletter\@ifundefined{FUM}{
\makeatletter\def\FUM{}
%%

\newcommand{\resp}{resp.\ }
\newcommand{\ifrac}[2]{#1/#2}
%% Quick typing
% \newcommand{\inv}{^{-1}}
\newcommand{\nm}[1]{{n-#1}}
\newcommand{\np}[1]{{n+#1}}

\newcommand{\mes}{{\textup{mes}}}

\newcommand{\bd}{\mathbf{d}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bZ}{\mathbb{Z}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bT}{\mathbb{T}}

\newcommand{\brA}{\bar{A}}
\newcommand{\brC}{\bar{C}}
\newcommand{\brrC}{\bar{\brC}}
\newcommand{\brrrC}{\bar{\brrC}}
\newcommand{\brn}{\bar{n}}
\newcommand{\brw}{\bar{w}}
\newcommand{\brW}{\overline{W}}
\newcommand{\brV}{\overline{V}}
\newcommand{\brx}{\bar{x}}
\newcommand{\breps}{\bar{\varepsilon}}
\newcommand{\brdelta}{\bar{\delta}}

\newcommand{\LC}{\mathbb{K}}
\newcommand{\LCt}{\widehat{\mathbb{K}}}

\newcommand{\cB}{\mathcal{B}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cR}{\mathcal{R}}

\newcommand{\hQ}{\widehat{Q}}
\newcommand{\hcR}{\widehat{\cR}}
\newcommand{\hx}{\widehat{x}}
\newcommand{\hdelta}{\widehat{\delta}}

\newcommand{\lboundary}{\partial^\text l}
\newcommand{\rboundary}{\partial^\text r}

\newcommand{\tcF}{\widetilde{\mathcal{F}}}
\newcommand{\tr}{\tilde{r}}
\newcommand{\tz}{\tilde{z}}

\newcommand{\matrixtt}[4]{\left(\begin{array}{cc}#1&#2\\#3&#4\end{array}\right)}
\newcommand{\vectt}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}
\newcommand{\Hcomp}{H-\hskip0pt component}
\newcommand{\Hcomps}{H-\hskip0pt components}

\newcommand{\ct}{r} % Collision time
\newcommand{\fft}{\tau} % Free flight time
\newcommand{\crit}{\textup{C}}
\newcommand{\ctc}{\ct_\crit}
\newcommand{\xc}{x_\crit}
\newcommand{\Uc}{\mathcal{U}_\crit}

\newcommand{\cm}{\mathcal{F}}
\newcommand{\cmp}{\hat\cm}
\newcommand{\cell}{\mathcal{D}}
\newcommand{\hol}{\mathcal{H}}
\newcommand{\recoPrivate}{\textup{R}}
\newcommand{\reco}{{\cell^-_{\recoPrivate}}}
\newcommand{\backReco}{{\cell^+_{\recoPrivate}}}
\newcommand{\recoMp}{{\cell^\mp_{\recoPrivate}}}
\newcommand{\redps}{\widetilde{\mathcal{M}}}
\newcommand{\exph}{\Omega}
\newcommand{\csp}{\mathcal{M}}
\newcommand{\cspi}{\widehat{\mathcal{M}}}
\newcommand{\csps}{\csp_\text{S}} % Reduced phase space of single collisions.
\newcommand{\invo}{\cI}
\newcommand{\flow}[1]{\Phi^{#1}} \newcommand{\rflow}[1]{\bar\Phi^{#1}}
\newcommand{\rell}{\bar\ell}
\newcommand{\reg}{\text{reg}}
\newcommand{\privateu}[1]{#1^*}
\newcommand{\privatel}[1]{#1_*}
\newcommand{\slope}{h}
\newcommand{\slopeb}{\mathfrak{h}}
\newcommand{\slopeu}{\privateu{\slope}} \newcommand{\slopel}{\privatel{\slope}}
\newcommand{\ellu}{\privateu{\ell}} \newcommand{\elll}{\privatel{\ell}}
\newcommand{\curv}{\kappa}
\newcommand{\cpar}{\mathcal{R}}
\newcommand{\pslope}{\mathcal{B}}
\newcommand{\cslope}{\mathcal{V}}
\newcommand{\aslope}{\tilde{\cslope}}
\newcommand{\Rect}{{\mathfrak{R}}}

\newcommand{\fixw}{\text{F}} \newcommand{\movw}{\text{M}}
\newcommand{\tang}{\mathcal{T}}
\newcommand{\tangu}{\mathcal{T}^1}

\newcommand{\unstable}{\text{u}}
\newcommand{\stable}{\text{s}}
\newcommand{\cone}{\mathcal{C}}
\newcommand{\conep}{\bar\cone^+}
\newcommand{\conen}{\bar\cone^-}
\newcommand{\coneu}{\cone^\unstable} \newcommand{\hconeu}{\hat{\cone}^\unstable} %fix with artillery
\newcommand{\cones}{\cone^\stable} \newcommand{\hcones}{\hat{\cone}^\stable}
\newcommand{\mconeu}{{\widetilde{\coneu}}}
\newcommand{\mcones}{{\widetilde{\cones}}}

\newcommand{\Ws}{W^{\stable}}
\newcommand{\Wu}{W^{\unstable}}
\newcommand{\dadm}[1]{\dadmPrivate^{#1}}
\newcommand{\dadmPrivate}{d\adm}
\newcommand{\deum}[1]{d\eum^{#1}}
\newcommand{\ds}{\dadmPrivate^{\stable}}
\newcommand{\du}{\dadmPrivate^{\unstable}}
\newcommand{\rs}{r_{\stable}}
\newcommand{\ru}{r_{\unstable}}

\newcommand{\eum}{_\text{E}}

\newcommand{\ppPrivate}[2]{#1^{#2}}
\newcommand{\prePrivate}[1]{\ppPrivate{#1}{-}}
\newcommand{\postPrivate}[1]{\ppPrivate{#1}{+}}
\newcommand{\prv}{\prePrivate{\bar v}}
\newcommand{\pov}{\postPrivate{\bar v}}
\newcommand{\prs}{\prePrivate{s}}
\newcommand{\pos}{\postPrivate{s}}
\newcommand{\prz}{\prePrivate{z}}
\newcommand{\poz}{\postPrivate{z}}
\newcommand{\prpslope}{\prePrivate{\pslope}}
\newcommand{\popslope}{\postPrivate{\pslope}}

% ** Singularities
\newcommand{\singPrivate}{\mathcal{S}}
\newcommand{\sing}[1]{\singPrivate^{#1}} % Singularities for \cm
\newcommand{\singp}[1]{\hat{\singPrivate}^{#1}} % Singularities for \cmp
\newcommand{\hsing}[1]{{\singPrivate}_\homo^{#1}} % Homo Singularities for \cm
\newcommand{\hsingp}[1]{\hat{\singPrivate}_\homo^{#1}} % Homo Singularities for \cm

\newcommand{\singReco}{\singPrivate_{\recoPrivate}}
\newcommand{\singBoth}{\singPrivate^\pm}
\newcommand{\singForward}[1]{\singPrivate^+_{#1}}
\newcommand{\singBackward}[1]{\singPrivate^-_{#1}}

\newcommand{\singt}[1]{\tilde{\singPrivate}^{#1}}
\newcommand{\singr}[1]{\sing{#1}_*}
\newcommand{\singrp}[1]{\singr{#1_*}}
\newcommand{\hhs}{\mathbb S}
\newcommand{\cE}{\mathcal E}
\newcommand{\cEs}{\mathcal E^{*}}

\newcommand{\nbhd}{\mathcal U}
\newcommand{\cc}{\hat Q}
\newcommand{\ccseq}[1]{\privSeq\cc{#1}}
\newcommand{\xseq}[1]{\privSeq x{#1}}
\newcommand{\indTuple}{\bar\indCell}

\newcommand{\admiss}{admissible}

\newcommand{\homo}{\mathbb{H}}
\newcommand{\homop}{\hat\homo}
\newcommand{\homosmall}{{\overline{\homo}}}
\newcommand{\kreg}{K^\text{reg}}
\newcommand{\zreg}{\cL^\text{reg}}
\newcommand{\ckreg}{\mathcal{K}^\text{reg}}
\newcommand{\ckregp}{\hat{\mathcal{K}}^\text{reg}}
\newcommand{\hkreg}{\hat{K}^\text{reg}}
\newcommand{\hzreg}{\hat{\cL}^\text{reg}}
\newcommand{\kregp}{\hkreg}
\newcommand{\kregtilde}{\tilde{K}^\text{reg}}
\newcommand{\largew}{w_*}
\newcommand{\cind}{\alpha}
\newcommand{\minB}{B_*}
\newcommand{\incB}{\beta}
\newcommand{\otherC}{\hat C}
\newcommand{\pme}{_\textup{p}}
\newcommand{\adm}{_{\alpha^{+}}}
\newcommand{\adms}{_{\alpha^{-}}}
\newcommand{\admPm}{_{\alpha^{\pm}}}
\newcommand{\admName}{\alpha^{+}}
\newcommand{\admNamePm}{\alpha^{\pm}}
\newcommand{\admNameM}{\alpha^{-}}
\newcommand{\aum}{_{*}}
\newcommand{\auum}{_{**}}
\newcommand{\admFunc}{\alpha^{+}}
\newcommand{\admFuncPm}{\alpha^{\pm}}
\newcommand\admParam[1]{%
  \ifnum0=#1\relax%
  \alpha_0
  \else%
  \ifnum1=#1\relax%
  \alpha_1\fi\fi}
\newcommand{\Np}{\hat N}
\newcommand{\cL}{\mathcal L}
\newcommand{\hcL}{\hat{\mathcal L}}
\newcommand{\rk}{\text{rank}}
\newcommand{\Leb}{\textup{Leb}}

\newcommand{\cQ}{\mathcal Q}
\newcommand{\cU}{\mathcal U}
\newcommand{\cV}{\mathbb V}
\newcommand{\sect}{\cV}
\newcommand{\nhbd}{\cU}
\newcommand{\qdrn}{\cQ}

\newcommand{\hlambda}{\hat\lambda}

\newcommand{\indCell}{\nu}
\newcommand{\redCell}{{\indCell^*}}
\newcommand{\multPrivate}{\mathcal{X}}
\newcommand{\mult}[1]{\multPrivate_{#1}}
\newcommand{\multp}[1]{\hat{\multPrivate}_{#1}}
\newcommand{\nb}[2]{\mathcal{U}_{#1,#2}}
\newcommand{\lft}{\textup{L}}
\newcommand{\rte}{\textup{R}}
\newcommand{\aft}{\textup{A}}
\newcommand{\bef}{\textup{B}}
\newcommand{\Const}{C_\#}
\newcommand{\Cdist}{C_\textup{D}}
\newcommand{\clo}{\text{cl}\,}
\newcommand{\privSeq}[2]{#1^{(#2)}}
\newcommand{\Wseq}[1]{\privSeq{W}{#1}}
\newcommand{\Wpseq}[1]{\privSeq{W'{}}{#1}}
\newcommand{\rgt}{\text{R}}
\newcommand{\Dom}{D}
\newcommand{\hDom}{\hat D}
\newcommand{\bA}{\mathbb A}
\newcommand{\nf}{\hat F}
\newcommand{\nfr}{\tilde F}
\newcommand{\bM}{M}
\newcommand{\prj}{\pi}
\newcommand{\tsl}[1]{T_{#1}}
\newcommand{\tj}{\tilde{\jmath}}
\newcommand{\tK}{\tilde{K}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\tx}{\tilde{x}}
\newcommand{\dn}{\nu}
\newcommand{\indexItinPrivate}[1]{^{(#1)}}
\newcommand{\dnt}[1]{\bar\nu\indexItinPrivate{#1}} %t stands for -tuple
\newcommand{\nt}[1]{\bar n\indexItinPrivate{#1}} %t stands for -tuple
\newcommand{\xit}[1]{\xi\indexItinPrivate{#1}}
\newcommand{\teta}{\tilde\eta}
\newcommand{\tetat}[1]{\teta\indexItinPrivate{#1}}
\newcommand{\LambdaMin}{\underline{\Lambda}}
\renewcommand{\deh}{d}

\newcommand{\If}{\boldsymbol{1}}
\newcommand{\expo}[1]{\exp(#1)}
\newcommand{\vn}{\vec n}

\newcommand{\hEs}{\hat E^{\stable}}
\newcommand{\hEu}{\hat E^{\unstable}}

\newcommand{\Cd}{C_{\textup{d}}}
\newcommand{\jac}[1]{\mathcal{J}_{#1}}
\newcommand{\jacW}{\jac{W}}
% \newcommand{\intr}{\text{int}\,}
}{} %%\@ifundefined{FUM}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

